Contract-Based Specification Refinement and Repair for Mission Planning

We address the problem of modeling, refining, and repairing formal specifications for robotic missions using assume-guarantee contracts. We show how to model mission specifications at various levels of abstraction and implement them using a library of pre-implemented specifications. Suppose the specification cannot be met using components from the library. In that case, we compute a proxy for the best approximation to the specification that can be generated using elements from the library. Afterward, we propose a systematic way to either 1) search for and refine the `missing part' of the specification that the library cannot meet or 2) repair the current specification such that the existing library can refine it. Our methodology for searching and repairing mission requirements leverages the quotient, separation, composition, and merging operations between contracts.

==> Tex/cgg.tex <==
\section{Enhanced Contract-Based Goal Graph}
\label{sec:cgg}

To model our graph of goals, we use the Contract-Based Goal Graph (CGG) ~\cite{mallozzi2020crome} and enhance it by making use of the contract merging operation. 
The CGG is a formal model that represents goals hierarchically. Each goal is mapped to one node of the CGG, and several nodes can be linked together in various ways.
 Formally, a CGG is a graph $T=(\Upsilon,\Xi)$, where each node $\upsilon \in \Upsilon$ is a goal and each \textit{directional} edge $\xi \in \Xi$ is a link that connects two goals together. We can have \textit{four} kinds of links: \textit{refinement}, \textit{composition}, \textit{conjunction} and \textit{merging}. A refinement link connects a goal to a more abstract one. The meaning associated with the other kinds of links are the following: all the incoming edges of the same kind of link in a node $n$ represent the goal nodes contributing to generating $n$ and the operation involved according to the link, i.e., composition, conjunction, or merging. 
 
 Automatic refinements can be produced by searching in a library of goals if any composition \textit{refines} the specification of any leaf-node of the CGG. 
 A library of goals is a set of goals $\Delta=\{\mathcal{L}_1, \mathcal{L}_2, \dots, \mathcal{L}_p\}$, with $p \in \mathbb{N}$. Every library goals is \textit{pre-implemented} in the sense that a finite-state machine that satisfies its specification has already been computed.
 
 

%  Whenever a refinement link is created, the assumptions resulting from the more refined goal will be automatically propagated in the more abstract goal and, by following the edges of the CGG, up to the root as detailed in~\cite{mallozzi2021incremental}. Assumption propagation makes sure that the refinements are always consistent, i.e., the set of assumptions of the refined goal must always be greater than or equal to those of the abstract goal (in the sense behaviour containment).
%  \pierg{maybe remove}




 \subsection{Generating the CGG}
The CGG represents the contextual robotic mission and is generated automatically from a set of goals. This paper introduces a different methodology to create a CGG with respect to~\cite{mallozzi2020crome} since we use a new contract operations.

We categorize goals in two \textit{viewpoints}: movement goals (e.g., visiting locations) and action goals (e.g., taking pictures, waving, etc.). Viewpoints can be interpreted as goals applied to different aspects of the same design. We use the contract operations of composition, conjunction, and merging as follows. 

\begin{itemize}
    \item \textbf{Conjunction} combines different mission scenarios. It is used to combine goals belonging to different mutually exclusive contexts. For example, we use conjunction to summarize into a single goal one goal from a daylight context and one goal that applies in the night.
 \item \textbf{Merging} is used to combine goals \textit{within a scenario} that belong to different viewpoints. For example, goals that concern the visit of locations can be merged with goals that prescribe the execution of actions.
 \item \textbf{Composition} is used to combine goals belonging to different objects in order to build a system. For example, the goals of two subsystems needed to implement a movement specification are composed.
\end{itemize}

% \pierg{TODO: add some discussion of why applying different contact operations is better than just do a conjunction of all the goals. e.g., conjunction of different context with different assumptions... combining same system/kinds vs different systems/kinds...}



==> Tex/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

\pierg{TODO: merge with discussion}
We presented a contract-based framework for modeling and refining robotic mission specifications using libraries of mission components at various abstraction layers. When the refinement of a specification is not possible out of the current library, we provided a method to automatically repair the specification, so that it can be refined using the library, or effectively guide the search for new implementations that can refine it. Our methodology is fully automated and based on contract manipulations via the quotient, separation, and merging operations. We implemented our framework in the tool \NAME. As future work, we plan to test it on a large-scale case study and further investigate the systematic generation of libraries for robotic mission specification.


% \pierg{TODO...}

% \pierg{TODO: write better}



%Finally, we maximize the reuse of the pre-implemented library of goals by choosing goals that cover the most number behaviors as possible so minimizing `missing behaviors' to be searched or used to repair.



% \iir{The conclusion talks too much about goals. We need to change the emphasis.}

==> Tex/related.tex <==
\section{Related Work}
\label{sec:related}
% \pierg{TODO: add/remove works and reorganize}\pierg{maybe leave only the specification repair section, which needs to be written better}


% \paragraph{Mission Specification}
% Various approaches have been proposed in the last years to specify missions. Some of them use logics~\cite{menghi2018multi,ulusoy2011optimal,fainekos2009temporal,guo2013revising,wolff2013automaton,kress2011robot,doi:10.1177/0278364914546174}.
% %and indeed they can be not the best solution in the case of end-users directly involved in the mission specification. 
% Other approaches make use of state charts~\cite{bohren2010smach,thomas2013new,klotzbucher2012coordinating} or Petri Nets~\cite{wang1991petri,ziparo2008petri}. 
% %and also, in this case, they require specialized knowledge and skills in their end-user. 
% To use such formalisms, the software engineer must have acquired skills in formal methods. 
% To make the mission specification more accessible, 
% %various researchers investigated and proposed domain-specific languages for mission specification
% various domain-specific languages for mission specification have been proposed, e.g., 
% \cite{GLRSWWCA12,campusano.ea:2017:live,DBLP:journals/corr/SchwartzNAM14,Ruscio2016,Bozhinoski2015,Ciccozzi4496,Doherty2012}.
% % The work in~\cite{dragule2021b} surveys domain-specific languages (DSLs) for robot mission specifications, classifies them into internal and external DSLs, and gives an overview of their tooling support. 
% Robotic patterns have been proposed as a solution to recurrent mission specification problems based on the analysis of mission requirements in the robotic literature~\cite{SpecificationPatternsTSE}. The PsALM tool~\cite{PSALM} enables the specification of robotic missions using mission specification patterns. \NAME supports $22$ patterns~\cite{SpecificationPatternsTSE}, capturing robot movements and actions performed as a robot moves in the environment. Robotic patterns help the designer formalize the contracts for each mission goal.


% \paragraph{Contract Refinement}
% In the context of contract-based verification, tools like OCRA~\cite{cimatti2013ocra} and AGREE~\cite{cofer2012compositional} use contracts to model system components and their aggregations and formally prove the correctness of contract refinements~\cite{cimatti2015contracts} by using model checkers~\cite{nuxmv}. 
% % \pierl{Le at al.~\cite{le2016contract} propose strategies to support modularization of requirements by contract decomposition.}
% Related to system engineering, CONDEnSe~\cite{ribeiro2019condense} propose a methodology and a tool that leverages the algebra of contracts to integrate artifacts developed in mechatronic systems.
% More oriented toward requirement engineering, the CHASE~\cite{nuzzo2018chase} framework combines a front-end formal specification language based on patterns with rigorous, contract-based verification and synthesis.
% In comparison with the works mentioned above, \NAME uses a hierarchical and incremental approach to refine contracts, leveraging on the modularity of the CGG and the reuse of goals from the library.


% \paragraph{Specification repair}
\pierg{TODO: move to intro}
Repairing of system specifications is a widely studied problem in the literature. Recent approaches have focused on repairing LTL specifications that are unrealizable for reactive synthesis~\cite{alur2013counter, cavezza2017interpolation, chatterjee2008environment, maoz2019symbolic, li2011mining}. These approaches focus on the discovery of \textit{new assumptions} to make the specification realizable. They use a restricted fragment of LTL specifications (e.g., GR(1)) and mostly use model checking techniques. More recent approaches by Gaaloul et al.~\cite{gaaloul2020mining} rely on testing rather than model checking to generate the data used to learn assumptions using machine learning techniques, and apply them to complex signal-based modeling notations rather than to LTL specifications. 
Brizio et al.~\cite{brizzio2021automated} use a search-based approach to repair LTL specifications. Their approach is based on syntactic and semantic similarity, where their heuristic is based on \textit{model counting}, i.e., the number of models that satisfy the formula. The new realizable specification is then produced by successive application of genetic operations. 
For repairing Signal Temporal Logic (STL) formulas, Gosh et al.~\cite{ghosh2016diagnosis} propose algorithms to detect possible reasons for infeasibility and suggest repairs to make it realizable. Approaches such as~\cite{ergurtuna2021automated, chatzieleftheriou2012abstract}, instead of repairing the specification, focus on repairing the \textit{system} in a way that it can satisfy the specification.
In the robotics domain, Boteanu et al.~\cite{pacheck2019automatic} focus on adding assumptions to the robot specification while having the human prompted to confirm or reject them. Pacheck et al.~\cite{pacheck2019automatic, pacheck2020finding} automatically encode into LTL formulas robot capabilities based on sensor data. If a task cannot be performed (i.e., the specification is unrealizable), they suggest skills that would enable the robot to complete the task.
% In the context of applying reactive synthesis for robotic specification Gazit...
% The idea to use library of components to meet high-level specifications is well established in the literature.\pierg{TODO: add works}
% The finding of missing components 

% Jing et al.~\cite{jing2016end} propose a system that uses requirements from a library of existing useful designs to meet high-level specification in the context of robotic application.
\pierg{TODO: add other related for library / missing component}



Our framework uses LTL specifications, but instead of mining for new assumptions or changing the system (i.e., the pre-implemented library goals), it repairs existing specifications (assumptions and guarantees) based on what can be refined from the library of goals. Our repairs are always the smallest (in terms of the behaviors removed from the original specification) and completely automated since they are based on algebraic operations. We use ideas similar to~\cite{brizzio2021automated} to compute the candidate composition, which is based on semantic and syntactic similarities to the goal to be refined.

% \iir{This only talks about repairing specs. We should say something about missing components. This problem has been extensively studied.}\pierg{i agree, i will also add more reference about realizing robotic missions via libraries}


% \pierg{other non-LTL, maybe remove}
% For repairing of Signal Temporal Logic (STL) formulas, Gosh et al.~\cite{ghosh2016diagnosis} propose algorithms to detect possible reasons for infeasibility and suggest repairs to make it realizable. Ergurtuna et al~\cite{ergurtuna2021automated} propose an automated framework to repair the \textit{system} that is violating an STL formula.
% For Computation Tree Logic (CTL) formulas, Chatzieleftheriou et al.~\cite{chatzieleftheriou2012abstract} propose changes in the model such that it satisfies a CTL formula. To avoid the state-explosion problem, their methodology uses model abstractions.




